Interaction is necessary for distributed learning with privacy or communication constraints

Local differential privacy (LDP) is a model where users send privatized data to an untrusted central server whose goal it to solve some data analysis task. In the non-interactive version of this model the protocol consists of a single round in which a server sends requests to all users then receives their responses. This version is deployed in industry due to its practical advantages and has attracted significant research interest. Our main result is an exponential lower bound on the number of samples necessary to solve the standard task of learning a large-margin linear separator in the non-interactive LDP model. Via a standard reduction this lower bound implies an exponential lower bound for stochastic convex optimization and specifically, for learning linear models with a convex, Lipschitz and smooth loss. These results answer the questions posed in \citep{SmithTU17,DanielyF18}. Our lower bound relies on a new technique for constructing pairs of distributions with nearly matching moments but whose supports can be nearly separated by a large margin hyperplane. These lower bounds also hold in the model where communication from each user is limited and follow from a lower bound on learning using non-adaptive \emph{statistical queries}.

==> MAJ-data-processing.tex <==
\section{Total variation distance and data processing inequality} \label{sec:tv}
\vitaly{This section should rather be omitted. }
\yuval{I am using the data processing inequality twice in different parts of the paper, but I feel like I shouldn't have it right in the preliminaries. What do you suggest doing?}
\vitaly{I think it's standard enough that most readers know it, and if needed can look it up easily. So there is no need to spell it out even in the prelims.}
\yuval{Still, I feel it's convenient to keep the data processing inequality here, so people can easily look it up, I guess not everyone is familiar with it.}
Let $P,Q$ be two probability distributions defined on the same probability space $(\Omega,\mathcal{F})$, where $\Omega$ is the sample space and $\mathcal{F}$ is the set of events. The \emph{total variation distance} between $P$ and $Q$ is defined as
\[
\dtv(P,Q) := \max_{F \in \mathcal{F}} |P(F) - Q(F)|.
\]
Given two spaces $(\Omega_1, \mathcal{F}_1)$ and $(\Omega_2, \mathcal{F}_2)$, a \emph{random function} $f$ from $\Omega_1$ to $\Omega_2$ is a function that given $a \in \Omega_1$, outputs a probability distribution $f_a$ over $\Omega_2$ (ignoring measurability issues). Given a probability distribution $P$ over $\Omega_1$, we define $f(P)$ as the probability distribution obtained by drawing $a \sim P$, drawing $b \sim f_a$ and then outputting $b$. We will use the standard \emph{data processing inequality} which states the following:
\begin{lemma}[Data processing inequality] \label{lem:data-processing}
	Let $P$ and $Q$ be two distributions over $\Omega_1$ and let $f$ be a measurable random function from $\Omega_1$ to $\Omega_2$. Then,
	\[
	\dtv(f(P),f(Q)) \le \dtv(P,Q).
	\]
\end{lemma}
%This lemma is intuitive: if $P$ and $Q$ are similar, applying the same transformation $f$ cannot make them different. 

==> MAJ-upper-bd.tex <==
\section{Upper bound}
\vitaly{This theorem used to be in the intro but I guess I've removed it at some point.}
We sketch the proof of Theorem~\ref{thm:upper}, starting with the second item. Assume without loss of generality that $f^*(x) = \mathbbm{1}_{x_1 \ge 0}$ and that any $x \in \supp(D)$ satisfies $\|x\|_2 = 1$.
We will draw independent vectors $\{w^{(1)},\dots,w^{(m)}\}$ from a normal multivariate Gaussian with zero mean and identity covariance, where $m = e^{O(\log(1/\epsilon)/\gamma^2)}$. For each vector $w^{(i)}$ we ask the statistical query $\err_{f_{w^{(i)}}}$, and select the function that minimizes this error.

For a random $w \sim N(0,I_n)$, we lower bound the probability that $\err_{f_{w}} \le \epsilon$. First, with probability $e^{-O(\log(1/\epsilon)/\gamma^2)}$ it holds that $w_{1} \ge \sqrt{2 \log (1/\epsilon)}/\gamma$. For any fixed $x \in \supp(D)$ it holds that $x_i f^*(x) \ge \gamma$, hence
\begin{align*}
\Pr_w\left[f_w(x) \ne  f^*(x) ~\middle|~ w_1 \ge \sqrt{2\log(1/\epsilon)}\right] \\
=\Pr_w\left[w^\top x f^*(x) \le 0 ~\middle|~ w_1 \ge \sqrt{2\log(1/\epsilon)}\right] \\
\le \Pr_w\left[ \sqrt{2 \log(1/\epsilon)} + (w_2,\dots,w_n)^\top(x_2,\dots,x_n)f^*(x) \le 0\right]\\
\le \epsilon,
\end{align*}
as $(w_2,\dots,w_n)^\top(x_2,\dots,x_n)f^*(x)$ is a Gaussian with mean zero and variance $\|(x_2, \dots, x_n)\|^2 \le 1$.
Taking expectation over $x \sim D$, we obtain that
\[
\E_w\left[\err_{f_w} ~\middle|~ w_1 \ge \sqrt{2\log(1/\epsilon)}\right]
\le \epsilon,
\]
therefore
\begin{align*}
\Pr_w\left[\err_{f_w} \le 2\epsilon \right] \\
\ge \Pr\left[\err_{f_w} \le 2\epsilon ~\wedge~ w_1 \ge \sqrt{2\log(1/\epsilon)}\right]\\
= \Pr\left[w_1 \ge \sqrt{2\log(1/\epsilon)}\right]
\Pr\left[\err_{f_w} \le 2\epsilon ~\middle|~ w_1 \ge \sqrt{2\log(1/\epsilon)}\right]\\
\ge e^{-O(\log(1/\epsilon)/\gamma^2)} \cdot 1/2.
\end{align*}
Hence, $e^{-O(\log(1/\epsilon)/\gamma^2)}$ random vectors suffice for getting a $w$ with classification error $2\epsilon$.

The proof of the first item is similar. We start by showing that with probability $e^{-O(\gamma^{-2a})}$, $w_1 \ge C\gamma^{-a}$ (where $C>0$ is a sufficiently large universal constant). Similar calculation shows that
\[
\E[\err_{f_w} \mid w_1 \ge C\gamma^{-a}] \le 1/2-\gamma^{1-a}.
\]
Hence,
\[
\Pr\left[\err_{f_w} \le 1/2-\gamma^{1-a}/2 \mid w_1 \ge C\gamma^{-a}\right]
\ge \Omega(1/\gamma^{1-a}).
\]
Hence, after drawing $e^{-O(\gamma^{-2a})}/\gamma^{1-a}$ random vectors $w$, one of them will have advantage $\Omega(\gamma^{1-a})$.

The third item of the proof follows from boosting \yuval{ref to smooth boosting}. The last item is a corollary of the previous items.

